Non-Clicks Mean Irrelevant? Propensity Ratio Scoring As a Correction

Recent advances in unbiased learning to rank (LTR) count on Inverse Propensity Scoring (IPS) to eliminate bias in implicit feedback. Though theoretically sound in correcting the bias introduced by treating clicked documents as relevant, IPS ignores the bias caused by (implicitly) treating non-clicked ones as irrelevant. In this work, we first rigorously prove that such use of click data leads to unnecessary pairwise comparisons between relevant documents, which prevent unbiased ranker optimization. Based on the proof, we derive a simple yet well justified new weighting scheme, called Propensity Ratio Scoring (PRS), which provides treatments on both clicks and non-clicks. Besides correcting the bias in clicks, PRS avoids relevant-relevant document comparisons in LTR training and enjoys a lower variability. Our extensive empirical evaluations confirm that PRS ensures a more effective use of click data and improved performance in both synthetic data from a set of LTR benchmarks, as well as in the real-world large-scale data from GMail search.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> backups/intro_Jan21_xuanhui.tex <==
\section{Introduction}
%1. implicit feedback for LTR, analysis (biased clicks lead to biased rankers: position bias, focus on those higher ranked relevant docs)
%2. Pairwise comparisons are most popular and easy, and widely used when binary labels. when using pairwise comparison for optimizing ranking metrics, only pairs with different labels contribute.
%3. IPS for unbised LTR -> unbiased ranking metric estimation. IPS only focus on clicked as relevant docs -> sub-optimal.
%4. In this work ...
Traditional retrieval systems rely on expert annotated relevance for learning to rank (LTR) model estimation. Even if possible to elicit, such explicit relevance labels are usually expensive to collect, not user-centric and non-evolving. This directly limits the application of LTR solutions in various scenarios, such as personal collection search \cite{wang2018pbe}.
In contrast, implicit feedback from users is an attractive alternative of relevance signals, free of aforementioned limitations. The most popularly used implicit feedback is user click data \cite{Joachims2002OSE}, which is often timely and cheap to collect at scale. 
Nevertheless, click data is also notoriously biased. 
%Nevertheless, it is notorious that the inherit biases in click data substantially weaken the capacity of obtaining an effective ranker \cite{Joachims2007Eval, Joachims2017interpretclick, yue2010beyondposition}. 
Most notably, the ranking order of documents in a result page (known as position bias) influences where the users would examine and click \cite{Joachims2017interpretclick}, e.g., higher ranked documents are more likely to be examined and clicked. Simply treating click/non-click as relevant/irrelevant substantially distorts LTR training \cite{Joachims2007Eval, Joachims2017interpretclick, yue2010beyondposition}.
%will lead to a ranker distracted from the relevance of documents and distorted by the position bias.  

%Recent research efforts apply counterfactual inference from observational studies \cite{Imbens2015causal} for unbiased LTR. 
Using Inverse Propensity Scoring (IPS) to debias implicit feedback, as introduced in \cite{joachims2017ips}, has made remarkable progress in unbiased LTR \cite{Agarwal2019GFC}. Specifically, by reweighing the clicked documents according to their propensities of being observed, IPS provides an unbiased estimate of the ranking metric of interest, such as Average Relevance Position (ARP, termed as $rank$ in \cite{joachims2017ips}). LTR is then achieved by empirical risk minimization based on the loss induced by this unbiased estimator. The induced loss is generally based on pairwise comparisons. For example, in a ranked list, clicked documents are either compared against all other documents to compute the rank loss as in propensity SVM-Rank \cite{joachims2017ips} or against unclicked documents as in Unbiased LambdaMART \cite{hu2019unbiasedlambda}.

Unfortunately, most unbiased LTR methods based on IPS \cite{wang2018pbe,ai2018DLA, joachims2017ips} can only correct bias in clicked documents. % since it is believed that only relevant documents contribute to the evaluation of ranking metrics. 
This can introduce a serious gap between the unbiased metric one expects to optimize and the actual loss one ends up with. The reason is straightforward but largely ignored by these methods: because non-click does not necessarily stand for irrelevance (e.g., it can be relevant but not examined), IPS inevitably includes the comparisons on relevant-relevant document pairs when forming the loss function with respect to clicks.  As a consequence, only reweighing clicked ones is insufficient to obtain an effective loss function for optimizing ranking metrics. 
%To comprehend the negative effect of such comparisons, we need to first thoroughly understand how LTR optimize ranking metrics in practice.
%
%However, IPS and most of its followup work \cite{wang2018pbe,ai2018DLA} only correct bias in clicked documents. Although it is believed that only relevant documents contribute to the evaluation of ranking metrics \cite{joachims2017ips}, such metrics have to be realized by pairwise comparisons between documents. For example, in a ranked list, clicked documents are either compared to all other documents to compute the rank loss in propensity SVM-Rank \cite{joachims2017ips} or unclicked documents in Unbiased LambdaMART \cite{hu2019unbiasedlambda}. As a result, only reweighing clicked ones is insufficient to make the resulting loss function unbiased. The reason is straightforward but largely ignored in unbiased LTR: because non-click does not necessarily stand for irrelevance, (e.g., it can be relevant but unexamined), IPS inevitably includes the comparisons on relevant-relevant document pairs, which introduces gap between the actual loss one optimizes and the unbiased loss one expects. To comprehend the negative effect of such comparisons, we need to first thoroughly understand the optimization of ranking metrics in practice.

% A ranking order is established by comparisons between documents.
%, each relevant documents must be compared to other documents in the ranked lists in order to calculate the ranking metrics. In particular, 
As shown in~\cite{Wang2018Lambdaloss}, for most popular ranking metrics, such as Average Relevance Position (ARP) used in \cite{joachims2017ips} and NDCG, % can be decomposed into pairwise comparisons.
%, where the order of a relevant document is counted by how many documents are scored higher than it. Most importantly, 
% The work points out that 
comparisons between pairs of the same relevance label only contribute a constant term to the ranking metric, regardless to their ranked positions or ranking scores. %~\cite{Wang2018Lambdaloss}. 
%In other words, only pairs with different relevance labels (e.g., relevant-irrelevant pairs in binary label case) have effects on the ranking metrics.
%This is the root cause of the optimization gap in IPS-based unbiased LTR, which introduces relevant-relevant comparisons when constructing the loss functions.  
%
Problems of IPS-based methods hence emerge when one constructs loss function based on the clicks. 
%Because the ranking metrics obtained from pairwise comparisons are discrete, thus not directly optimizable, continuous approximations are often used bound the metric for optimization, %which is the underlying principles of utilizing pairwise losses for optimizing ranking metrics, usually 
%also known as pairwise LTR \cite{Joachims2002OSE,Arias2008logistic,burges2010lambdamart}. 
% As previously discussed, 
Loss should only be counted on pairs with different relevance labels, since the other pairs do not affect the ranking metric and therefore do not contribute to the loss. Nevertheless, IPS can only revealing relevance of clicked documents; there is no guarantee that each clicked document is only compared to truly irrelevant documents. Consequently, IPS-based LTR methods impose losses on relevant-relevant pairs, which distort the true objective and lead to sub-optimal results. 

From a more intuitive perspective, we can decompose the click data as in Figure \ref{fig:clickdata}. In noise-free setting, only when relevant document is observed, it will be clicked. Those relevant but uncliked documents are mistakenly used as negative examples and have no chance to be explicitly promoted, resulting in rankers still biased to them. This could also be indicated by the empirical observation that only when there is little bias can the performance of IPS be guaranteed \cite{Jagerman2019modelorintervene}. Because strong bias could conceal lots of relevant documents in unclicked documents. Thus it is crucial to remove the relevant documents from negative examples, which can be realized by identifying truly irrelevant documents from unclicked documents for effective comparisons. Hoewever, one important property of the click data is that only positive feedback (i.e., clicks) is logged. There is no negative feedback. As shown in Figure \ref{fig:clickdata}, unclicked documents are not necessarily observed irrelevance labels, which is \emph{asymmetric} to clicks. Hence, IPS is not applicable to reveal the irrelevant documents from non-clicks. Despite the attempts of debiasing the unclicked documents in a similar manner to clicked documents \cite{hu2019unbiasedlambda}, the assumption that non-click probability is proportional to the irrelevant probability does not hold. %In particular, non-clicks contain both observed and unobserved documents, \emph{asymmetric} to clicks that must be based upon observation. 
Specific treatments on unclicked documents are necessary. 

In this work, we propose a principled framework called Propensity Ratio Scoring (PRS) for unbiased LTR with pairwise comparisons, which addresses the above problems. We first theoretically prove that IPS based on pairwise comparisons include losses that do not contribute to the ranking metric, resulting in a gap to the true objective of our interest. In order to construct valid pairs to promote relevant documents for unbiased LTR, we introduce treatments on both clicked  and unclicked documents. In particular, we first debias the clicks for representing the relevance, which could be achieved from IPS. Second, to avoid the mistake of using relevant but unclicked documents as negative examples, we also identifie the truly irrelevant documents from unclicked documents to compare to each clicked document. %Our key insight is that under noise-free setting, if a document is observed (examined), click/non-click is equivalent to relevance/irrelevance. Reversely, if a document is unclicked but observed, it indicates true irrelevance. 
We develop PRS with both theoretical and empirical justifications step-by-step, and show that PRS inspires a more effective use of click data with reduced variance. As there is no specific heuristics needed, it can be seamlessly generalized to various unbiased LTR settings (e.g., different click propensity models, different learning algorithms, joint learning of propensities and rankers) and even other scenarios (e.g., recommendation \cite{Schnabel2016RecTreat}). We conduct comprehensive empirical evaluations based on benchmark datasets, which demonstrate the superior performance of the proposed solution. %Furthermore, we also preform real-world experiments by building an extension on Chrome....    

%Besides, preliminary estimation of the position-based propensities are assumed for applying IPS \cite{wang2018pbe,Agarwal2019EPB}. Although there are works that extend the the IPS framework to jointly estimate the propensities and the unbiased ranker \cite{ai2018DLA, hu2019unbiasedlambda}, the feasibility and performance guarantees lack necessary theoretical justifications. In this work, we keep the separation of the propensity estimation and learning new rankers as in \cite{joachims2017ips,wang2018pbe}, and concentrate on the principled foundations of unbiased LTR. 


==> backups/intro_jan20.tex <==
\section{Introduction}
%1. implicit feedback for LTR, analysis (biased clicks lead to biased rankers: position bias, focus on those higher ranked relevant docs)
%2. Pairwise comparisons are most popular and easy, and widely used when binary labels. when using pairwise comparison for optimizing ranking metrics, only pairs with different labels contribute.
%3. IPS for unbised LTR -> unbiased ranking metric estimation. IPS only focus on clicked as relevant docs -> sub-optimal.
%4. In this work ...
Traditional retrieval systems rely on expert annotated relevance for learning to rank (LTR) model estimation. Even if possible to elicit, such explicit relevance labels are usually expensive to collect, not user-centric and non-evolving. This directly limits the applicability LTR solutions in various scenarios, such as personal collection search \cite{wang2018pbe}.
In contrast, implicit feedback from searchers is an attractive source of relevance signals free of aforementioned limitations. The most popularly used implicit feedback is user click data \cite{Joachims2002OSE}, which is often abundant, timely, and easy to collect. 
Nevertheless, click data is also notoriously biased. 
%Nevertheless, it is notorious that the inherit biases in click data substantially weaken the capacity of obtaining an effective ranker \cite{Joachims2007Eval, Joachims2017interpretclick, yue2010beyondposition}. 
Most notably, the ranking order of documents in a result page (known as position bias) influences where the user would examine and click \cite{Joachims2017interpretclick}, e.g., higher ranked documents are more likely to be examined and clicked. Simply treating click/non-click as relevant/irrelevant substantially distorts LTR training \cite{Joachims2007Eval, Joachims2017interpretclick, yue2010beyondposition}.
%will lead to a ranker distracted from the relevance of documents and distorted by the position bias.  

Recent research efforts in debiasing the click data for LTR stem from counterfactual inference for observational studies \cite{Imbens2015causal}. Using Inverse Propensity Scoring (IPS) for debiasing implicit feedback as introduced in \cite{joachims2017ips} has made remarkable progress for unbiased LTR \cite{Agarwal2019GFC}. Specifically, based on the revealed relevance labels from clicked documents, IPS provides an unbiased estimate of the ranking metric of interest, such as rank \cite{joachims2017ips}. The learning of a new ranker is then achieved by empirical risk minimization based on the unbiased estimator. 

\begin{comment}
However, one important property of click data is that merely positive feedback (i.e., clicks) is logged, while there is no recorded negative feedback. This fact restricts the application of IPS to only \emph{clicked} documents in a pointwise sense. As unclicked documents are not necessarily observed, IPS is not able to distinguish the \emph{truly} irrelevant documents from unclicked documents. Although it is argued that clicks are sufficient because only relevant documents contribute to the ranking metrics \cite{joachims2017ips}, it is impossible to obtain the ranking metric with only relevant documents but without negative examples. %Although it is argued that clicks are sufficient to get an unbiased estimate of the ranking metrics which are mostly defined on relevant documents \cite{joachims2017ips}, it is impossible to obtain the ranking metric with only relevant documents but without negative examples.
%such ranking metrics obtained from the IPS estimator are not directly optimizable.

As ranking order is derived by comparisons between documents, each relevant documents must be compared to other documents in the ranked lists in order to calculate the ranking metrics. In particular, as shown in~\cite{Wang2018Lambdaloss}, popular metrics such as Average Relevance Position (ARP) used in \cite{joachims2017ips} and NDCG can be decomposed into pairwise comparisons, so that the rank of a relevant document could be counted by how many documents are scored higher than it. When the ranking metrics are achieved with such pairwise comparisons, it has been proved that pairs with the same labels will form a constant term in the ranking metric, regardless to their ranked positions or ranking scores~\cite{Wang2018Lambdaloss}. On the other hand, this indicates that only pairs with different labels (relevant-irrelevant pairs in binary label case) have effects on the ranking metrics. %\xw{I made some derivation. I think the relevant-relevant pairs will contribute a constant term to the metrics, no matter there scores are. However, when we set a pair of losses such as logistic losses on these pairs, the sum of the pairs of losses would prefer that the two relevant documents to have the same scores -- which is not necessary and leads to a sub optimal results for the ranking metrics.}

%Applications of IPS usually focus on \emph{clicked} documents in a pointwise sense. The underlying idea is that only \emph{relevant} documents contribute to the unbiased estimate of the ranking metric \cite{joachims2017ips}. When LTR tasks are achieved from pairwise comparisons, which has been proved to be more effective and popularly applied, relevant documents are promoted by comparing to \emph{irrelevant} documents \cite{Joachims2002OSE}. However, IPS is only applicable for recovering the objective defined on relevant documents from clicks, because clicked documents are both observed and relevant (i.e., click probability is proportional to the relevance probability). Due to the fact that we do not know the reason of a non-click (either the document is unobserved or irrelevant or both) \cite{ai2018DLA}, IPS is not able to distinguish the \emph{truly} irrelevant documents from unclicked documents. Despite the attempts of debiasing the unclicked documents in a similar manner to clicked documents \cite{hu2019unbiasedlambda}, the assumption that non-click probability is proportional to the irrelevant probability does not hold.  

%Pairwise LTR methods ranging from basic pairwise logistic regression \cite{Arias2008logistic,rendle2009bpr} to the state-of-the-art algorithms like LambdaMART \cite{burges2010lambdamart} are widely studied and applied due to their advantages of promising performance and ease of use. When relying on pairwise comparisons to optimize ranking metrics as in Rank SVM \cite{Joachims2002OSE}, one can theoretically prove that only pairs with different labels (relevant-irrelevant pairs in binary label case) contribute to the optimization \cite{Wang2018Lambdaloss}. 
Besides, the ranking metrics obtained from pairwise comparisons are discrete, and thus not directly optimizable. Continuous approximations are needed to bound the metric for optimization, which is the underlying principles of using pairwise losses for optimizing ranking metrics, known as pairwise LTR \cite{Joachims2002OSE,Arias2008logistic,burges2010lambdamart}. As previously discussed, only pairs with different labels have effects on the ranking metrics. Therefore, when approximating the results of pairwise comparisons, only pairwise losses imposed on pairs with different labels can contribute to the optimization. For example, the loss on relevant-relevant pairs are invalid to optimizing the ranking metric. Nevertheless, IPS based LTR methods are only designed for revealing relevance of documents from clicks. When formulating pairs with click data, each clicked document is compared to either unclicked documents (e.g., Unbiased LambdaMart \cite{hu2019unbiasedlambda}), or all other documents (e.g., Propensity SVM-Rank \cite{joachims2017ips}). As non-click does not necessarily mean irrelevant (e.g., relevant but unobserved documents are also not clicked), there is no guarantee that each clicked document is compared to truly irrelevant documents. Therefore, pairwise based IPS estimators include losses on relevant-relevant pairs, which dilute the true objective and lead to sub-optimal results. From a more intuitive perspective, those relevant but uncliked documents are mistakenly used as negative examples and have no chance to be explicitly promoted, resulting in rankers still biased to them. This could also be indicated by the empirical observation that only when there is little bias can the performance of IPS be guaranteed \cite{Jagerman2019modelorintervene}. Because strong bias could conceal lots of relevant documents in unclicked documents. Thus it is crucial to remove the relevant documents from negative examples, which can be realized by identifying truly irrelevant documents from unclicked documents for effective comparisons. Despite the attempts of debiasing the unclicked documents in a similar manner to clicked documents \cite{hu2019unbiasedlambda}, the assumption that non-click probability is proportional to the irrelevant probability does not hold. 
In particular, non-clicks contain both observed and unobserved documents, \emph{asymmetric} to clicks that must be based upon observation. Specific treatments on unclicked documents are necessary. 
\end{comment}  

In this work, we propose a principled framework called Propensity Ratio Scoring (PRS) for unbiased LTR with pairwise comparisons, which addresses the above problems. We first theoretically prove that IPS based on pairwise comparisons include losses that do not contribute to the ranking metric, resulting in a gap to the objective of our interest. In order to construct valid pairs to promote relevant documents for unbiased LTR, we imposes proper treatments on both clicked documents and unclicked documents. In particular, we first debias the clicks for representing the relevance, which could be achieved from IPS. Second, to avoid the mistake of using relevant but unclicked documents as negative examples, we also identifie the truly irrelevant documents from unclicked documents to compare to each clicked document. %Our key insight is that under noise-free setting, if a document is observed (examined), click/non-click is equivalent to relevance/irrelevance. Reversely, if a document is unclicked but observed, it indicates true irrelevance. 
We develop PRS with both theoretical and empirical justifications step-by-step, and show that PRS inspires a more effective use of click data with reduced variance. As there is no specific heuristics needed, it can be seamlessly generalized to various unbiased LTR settings (e.g., different click propensity models, different learning algorithms, joint learning of propensities and rankers) and even other scenarios (e.g., recommendation \cite{Schnabel2016RecTreat}). We conduct comprehensive empirical evaluations based on benchmark datasets, which demonstrate the superior performance of the proposed solution. %Furthermore, we also preform real-world experiments by building an extension on Chrome....    

%Besides, preliminary estimation of the position-based propensities are assumed for applying IPS \cite{wang2018pbe,Agarwal2019EPB}. Although there are works that extend the the IPS framework to jointly estimate the propensities and the unbiased ranker \cite{ai2018DLA, hu2019unbiasedlambda}, the feasibility and performance guarantees lack necessary theoretical justifications. In this work, we keep the separation of the propensity estimation and learning new rankers as in \cite{joachims2017ips,wang2018pbe}, and concentrate on the principled foundations of unbiased LTR. 


==> backups/intro_jan21.tex <==
\section{Introduction}
%1. implicit feedback for LTR, analysis (biased clicks lead to biased rankers: position bias, focus on those higher ranked relevant docs)
%2. Pairwise comparisons are most popular and easy, and widely used when binary labels. when using pairwise comparison for optimizing ranking metrics, only pairs with different labels contribute.
%3. IPS for unbised LTR -> unbiased ranking metric estimation. IPS only focus on clicked as relevant docs -> sub-optimal.
%4. In this work ...
Traditional retrieval systems rely on expert annotated relevance for learning to rank (LTR) model estimation. Even if possible to elicit, such explicit relevance labels are usually expensive to collect, not user-centric and non-evolving. This directly limits the application of LTR solutions in various scenarios, such as personal collection search \cite{wang2018pbe}.
In contrast, implicit feedback from users is an attractive alternative of relevance signals, free of aforementioned limitations. The most popularly used implicit feedback is user click data \cite{Joachims2002OSE}, which is often  timely and cheap to collect at scale. 
Nevertheless, click data is also notoriously biased. 
%Nevertheless, it is notorious that the inherit biases in click data substantially weaken the capacity of obtaining an effective ranker \cite{Joachims2007Eval, Joachims2017interpretclick, yue2010beyondposition}. 
Most notably, the ranking order of documents in a result page (known as position bias) influences where the users would examine and click \cite{Joachims2017interpretclick}, e.g., higher ranked documents are more likely to be examined and clicked. Simply treating click/non-click as relevant/irrelevant substantially distorts LTR training \cite{Joachims2007Eval, Joachims2017interpretclick, yue2010beyondposition}.
%will lead to a ranker distracted from the relevance of documents and distorted by the position bias.  

%Recent research efforts apply counterfactual inference from observational studies \cite{Imbens2015causal} for unbiased LTR. 
Using Inverse Propensity Scoring (IPS) to debias implicit feedback, as introduced in \cite{joachims2017ips}, has made remarkable progress in unbiased LTR \cite{Agarwal2019GFC}. Specifically, by reweighing the clicked documents according to their propensities of being observed, IPS provides an unbiased estimate of the ranking metric of interest, such as rank \cite{joachims2017ips}. LTR is then achieved by empirical risk minimization based on the loss induced by this unbiased estimator. 
However, most unbiased LTR methods based on IPS \cite{wang2018pbe,ai2018DLA} only correct bias in clicked documents, since it is believed that only relevant documents contribute to the evaluation of ranking metrics \cite{joachims2017ips}. But this unfortunately introduces a serious gap between the unbiased loss one expects to optimize and the actual loss one ends up with. The reason is straightforward but largely ignored in IPS: because non-click does not necessarily stand for irrelevance (e.g., it can be relevant but unexamined), IPS inevitably includes the comparisons on relevant-relevant document pairs when forming the loss function with respect to clicks. For example, in a ranked list, clicked documents are either compared against all other documents to compute the rank loss in propensity SVM-Rank \cite{joachims2017ips} or against unclicked documents in Unbiased LambdaMART \cite{hu2019unbiasedlambda}. As a consequence, only reweighing clicked ones is insufficient to make the resulting loss function unbiased. To comprehend the negative effect of such comparisons, we need to first thoroughly understand the optimization of ranking metrics in practice.
%However, IPS and most of its followup work \cite{wang2018pbe,ai2018DLA} only correct bias in clicked documents. Although it is believed that only relevant documents contribute to the evaluation of ranking metrics \cite{joachims2017ips}, such metrics have to be realized by pairwise comparisons between documents. For example, in a ranked list, clicked documents are either compared to all other documents to compute the rank loss in propensity SVM-Rank \cite{joachims2017ips} or unclicked documents in Unbiased LambdaMART \cite{hu2019unbiasedlambda}. As a result, only reweighing clicked ones is insufficient to make the resulting loss function unbiased. The reason is straightforward but largely ignored in unbiased LTR: because non-click does not necessarily stand for irrelevance, (e.g., it can be relevant but unexamined), IPS inevitably includes the comparisons on relevant-relevant document pairs, which introduces gap between the actual loss one optimizes and the unbiased loss one expects. To comprehend the negative effect of such comparisons, we need to first thoroughly understand the optimization of ranking metrics in practice.

A ranking order is obtained by comparisons between documents.
%, each relevant documents must be compared to other documents in the ranked lists in order to calculate the ranking metrics. In particular, 
As shown in~\cite{Wang2018Lambdaloss}, most popular ranking metrics, such as Average Relevance Position (ARP) used in \cite{joachims2017ips} and NDCG, can be decomposed into pairwise comparisons, where the order of a relevant document is counted by how many documents are scored higher than it. The work also proves that comparisons between pairs of the same relevance labels contribute a constant term in the ranking metric, regardless their ranked positions or ranking scores~\cite{Wang2018Lambdaloss}. % In other words, only pairs with different relevance labels (e.g., relevant-irrelevant pairs in binary label case) contribute to the ranking metrics.
This is the root cause of the optimization gap in IPS-based unbiased LTR, which introduces relevant-relevant comparisons when constructing the loss functions.  

Furthermore, the ranking metrics obtained from pairwise comparisons are discrete, and thus not directly optimizable. Continuous approximations are needed to bound the metric for optimization, %which is the underlying principles of utilizing pairwise losses for optimizing ranking metrics, usually 
known as pairwise LTR \cite{Joachims2002OSE,Arias2008logistic,burges2010lambdamart}. As discussed, only pairs with different relevance labels affect the ranking metrics. Therefore, when approximating the results of pairwise comparisons, only pairwise losses imposed on pairs with different labels should contribute to the optimization. For example, the loss on relevant-relevant pairs are invalid to optimizing the ranking metric. Nevertheless, IPS-based LTR methods are only designed for revealing relevance of documents from clicks. There is no guarantee that each clicked document is compared to truly irrelevant documents. Consequently, IPS based LTR methods include losses on relevant-relevant pairs, which dilute the true objective and lead to sub-optimal results. 

From a more intuitive perspective, we can decompose the click data as in Figure \ref{fig:clickdata}. In noise-free setting, only when relevant document is observed, it will be clicked. Those relevant but uncliked documents are mistakenly used as negative examples and have no chance to be explicitly promoted, resulting in rankers still biased to them. This could also be indicated by the empirical observation that only when there is little bias can the performance of IPS be guaranteed \cite{Jagerman2019modelorintervene}. Because strong bias could conceal lots of relevant documents in unclicked documents. Thus it is crucial to remove the relevant documents from negative examples, which can be realized by identifying truly irrelevant documents from unclicked documents for effective comparisons. Hoewever, one important property of the click data is that only positive feedback (i.e., clicks) is logged. There is no negative feedback. As shown in Figure \ref{fig:clickdata}, unclicked documents are not necessarily observed irrelevance labels, which is \emph{asymmetric} to clicks. Hence, IPS is not applicable to reveal the irrelevant documents from non-clicks. Despite the attempts of debiasing the unclicked documents in a similar manner to clicked documents \cite{hu2019unbiasedlambda}, the assumption that non-click probability is proportional to the irrelevant probability does not hold. %In particular, non-clicks contain both observed and unobserved documents, \emph{asymmetric} to clicks that must be based upon observation. 
Specific treatments on unclicked documents are necessary. 

In this work, we propose a principled framework called Propensity Ratio Scoring (PRS) for unbiased LTR with pairwise comparisons, which addresses the above problems. We first theoretically prove that IPS based on pairwise comparisons include losses that do not contribute to the ranking metric, resulting in a gap to the true objective of our interest. In order to construct valid pairs to promote relevant documents for unbiased LTR, we introduce treatments on both clicked  and unclicked documents. In particular, we first debias the clicks for representing the relevance, which could be achieved from IPS. Second, to avoid the mistake of using relevant but unclicked documents as negative examples, we also identifie the truly irrelevant documents from unclicked documents to compare to each clicked document. %Our key insight is that under noise-free setting, if a document is observed (examined), click/non-click is equivalent to relevance/irrelevance. Reversely, if a document is unclicked but observed, it indicates true irrelevance. 
We develop PRS with both theoretical and empirical justifications step-by-step, and show that PRS inspires a more effective use of click data with reduced variance. As there is no specific heuristics needed, it can be seamlessly generalized to various unbiased LTR settings (e.g., different click propensity models, different learning algorithms, joint learning of propensities and rankers) and even other scenarios (e.g., recommendation \cite{Schnabel2016RecTreat}). We conduct comprehensive empirical evaluations based on benchmark datasets, which demonstrate the superior performance of the proposed solution. %Furthermore, we also preform real-world experiments by building an extension on Chrome....    

%Besides, preliminary estimation of the position-based propensities are assumed for applying IPS \cite{wang2018pbe,Agarwal2019EPB}. Although there are works that extend the the IPS framework to jointly estimate the propensities and the unbiased ranker \cite{ai2018DLA, hu2019unbiasedlambda}, the feasibility and performance guarantees lack necessary theoretical justifications. In this work, we keep the separation of the propensity estimation and learning new rankers as in \cite{joachims2017ips,wang2018pbe}, and concentrate on the principled foundations of unbiased LTR. 


==> backups/method-Aug11.tex <==
\section{The Issue of Inverse Propensity Scoring in Practice}
In this section, we first formally formulate the problem of unbiased LTR and the general theory of IPS. % to set up the foundation for analysis, whose objective is to optimize ranking metrics with biased implicit feedback. 
Then based on an in-depth discussion of practical ranking metrics optimization, we elaborately investigate and disclose the deficiency of IPS in solving the problem. 

\subsection{Unbiased Learning to Rank}
\label{sec:unbiaLTR}
Without loss of generality, in LTR tasks we are given a set of i.i.d. queries $\bm{Q}$, where each query instance $q$ is sampled from an underlying distribution $q \sim P(q)$. Suppose we have a ranking system $S$, which generates a ranked list of documents $\pi_q$ retrieved for each query $q$. The order in $\pi_q$ is typically derived from the predicted \emph{relative} relevance values (or ranking scores) by $S$. Then the empirical risk $\mathcal{R}$ on $S$ is computed as:
\begin{equation*}
    \mathcal{R}(Q, S) = \frac{1}{|\bm Q|}\sum_{q\in\bm Q}R(\pi_q|q).
\end{equation*}
As the queries are independent and query-level analysis is not our focus in this work, we concentrate on the local risk from a single query $q$. Specifically, denote the relevance vector for all documents to query $q$ as $r_q$; and the ranked list $\pi_q$ is obtained by the predicted relevance values $\hat r_q$ by $S$. Let $x_i$ be a document in the ranked list, and $r_q(x_i)$ be the ground-truth relevance label of $x_i$ under query $q$. To simplify our discussion, assume the relevance label is binary, i.e., $r_q(x_i)\in \{0,1\}$. The goal of LTR is to optimize the ranking metric of our interest (e.g., ARP, NDCG, MAP, etc). Thus the local risk incurred on a query is defined on the ranking metric calculated on $\pi_q$. When the ranking metric is defined on relevant documents as in most cases \cite{joachims2017ips,ai2018DLA}, we can decompose the local risk as:
\begin{equation}
    R(\pi_q|q) = \sum_{x_i:r_q(x_i)=1}\Delta(x_i|\pi_q)
\end{equation}
where $\Delta(x_i|\pi_q)$ is the individual contribution from a relevant document $x_i$ to the ranking metric, e.g., the $rank$ of $x_i$ in ARP or the discounted gain of $x_i$ in NDCG. 

Unlike the full-information setting where the relevance labels of all documents in $\pi_q$ are known, $r_q$ is only partially observed in the implicit click feedback. 
In particular, the examination model \cite{richardson2007predicting} asserts that a user has to first examine a document to observe its relevance label before he/she decides to click it based on the relevance. Most relevance labels may remain unobserved. For example, given a presented ranking $\tilde\pi_q$, the relevance labels on the top-ranked documents are more likely to be observed than those on the lower-ranked positions, known as the position  bias \cite{wang2018pbe,Craswell2008clickpositionbias}. Following the counterfactual model introduced in \cite{joachims2017ips}, denote $o_q$ as a 0/1 vector indicating whether the relevance labels in $r_q$ are observed. For each element of $o_q$, the marginal probability $P(o_q(x_i)=1|\tilde\pi_q)$ of observing the relevance label $r_q(x_i)$ in $\tilde\pi_q$ is referred as the observation propensity of document $x_i$. Consider the deterministic noise-free setting in \cite{joachims2017ips}, %where examination of a document is equal to the observation of its relevance label. A
a document is clicked if and only if it is examined (thus observed) and relevant, i.e., $c_q(x_i)\Leftrightarrow o_q(x_i)\wedge r_q(x_i)$, while all other documents are recorded as unclicked. Note that an important property of click data is that only the positive feedback is logged, i.e., clicks. When a document is not clicked, it is unknown if it is irrelevant or not observed, as illustrated in Figure \ref{fig:clickdata}.
%This means even an irrelevance label is observed, it is not recorded in the implicit feedback. 
To be more explicit, we use another binary vector $c_q$ to denote whether each document is clicked under $q$. 

%Consider the deterministic noise-free setting in \cite{joachims2017ips}, where examination of a document is equal to the observation of its relevance label. A document is clicked if and only if it is observed and relevant, i.e., $c_q(x_i)\Leftrightarrow o_q(x_i)\wedge r_q(x_i)$, while all other documents are recorded as unclicked. As shown in Figure \ref{fig:clickdata}, the click data can be decomposed based on each document's true relevance label and whether it is observed. The unclicked documents are composed of irrelevant documents (both observed or unobserved) as well as relevant but unobserved documents. %There is no negative feedback.
%i.e., when the a relevant document is observed, it is clicked,  In Figure \ref{fig:clickdata}, we decompose the click data based on each document's relevance and whether the relevance label is observed. As is illustrated, the unclicked documents is composed with irrelevant documents (both observed or unobserved) as well as relevant but unobserved documents. There is no explicit negative feedback.  Specifically, we use another 0/1 vector $c_q$ to denote whether each document is clicked. 

Under this setting, given the clicks in a logged ranking $\tilde\pi_q$, we can get an unbiased estimate of $R(\pi_q|q)$ for any new ranking $\pi_q$ with the IPS estimator \cite{Imbens2015causal,Paul1983central}:
\begin{align}
\label{eq:IPS}
    R_{IPS}(\pi_q|q,\tilde\pi_q,o_q) &= \sum_{x_i:c_q(x_i)=1}\frac{\Delta(x_i|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)} \\\nonumber
    &= \mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge\; r_q(x_i)=1}\frac{\Delta(x_i|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
It has been proved that $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ provides an unbiased estimate of $R(\pi_q|q)$ for any new ranking $\pi_q$: $E_{o_q}[R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)]\\=R(\pi_q|q)$ \cite{joachims2017ips}. Thus optimizing $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ will lead to the same ranker as from $R(\pi_q|q)$, in terms of expectation. 

\subsection{Ranking Metrics Optimization}
\label{sec:metric-optimization}
Note that $R(\pi_q|q)$ and $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ are discrete metrics on relevant documents in a pointwise sense and are not directly optimizable \cite{Christopher2007nonsmooth}. In order to practically optimize the ranking metrics, we need to explicitly calculate the metric on a ranking $\pi_q$ and formulate the optimizable loss with continuous approximations. Our analysis of the deficiency of IPS is based on the following two arguments of practical ranking metrics optimization. 

%$R(\pi_q|q)$ and $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ are discrete metrics on relevant documents. They are not directly optimizable even with fully labeled relevance judgements \cite{Christopher2007nonsmooth}. In order to practically optimize the ranking metrics, we need to first calculate the metric on a ranking $\pi_q$ and reformulate the risk with continuous approximations.

Firstly, the individual contribution $\Delta(x_i|\pi_q)$ of a relevant document has to be obtained from its comparisons to other documents in the ranking list $\pi_q$, as the ranking position of $x_i$ in $r_q$ depends on how many other documents are predicted to be more relevant than $x_i$ by $S$. As is shown in \cite{Wang2018Lambdaloss}, this could be realized via pairwise comparisons for a set of general ranking metrics. For instance, to get the $rank$ of a relevant document $x_i$ in $\pi_q$, we need to compare the predicted relevance between $\hat r_q(x_i)$ to each other document's $\hat r_q(x_j)$. One important property in such pairwise formulation is that the comparisons between two documents of the \emph{same} label will form a constant term in the ranking metric, agnostic to their positions or predicted relevance values \cite{Wang2018Lambdaloss}. Hence, only the comparisons between documents with \emph{different} labels affect the ranking metrics and therefore can contribute to the optimization. 

Secondly, the resulting metrics are discrete. Thus continuous approximations such as logistic loss \cite{Arias2008logistic} or hinge loss \cite{Joachims2002OSE} are needed for practical optimization. %For example, logistic loss \cite{Arias2008logistic} or hinge loss \cite{Joachims2002OSE} are typical approximations for pairwise comparisons that bound the ranking metric of our interest. Equivalently, one can also introduce the approximations on the gradient of the metric from pairwise comparisons, such as the lambda loss \cite{burges2010from, Wang2018Lambdaloss}. 
Based on the first point, the pairwise loss should be imposed \emph{only} on the document pairs with different labels, which can really contribute to the ranking metric optimization. Imposing loss on document pairs with the same label will introduce extra irreducible terms in the total loss that distorts the optimization and leads to sub-optimal results. 

To theoretically and explicitly illustrate our claims, we take the optimization of Average Relevance Position (ARP) used in the original analysis of IPS \cite{joachims2017ips} as an example. Assume there are $n$ documents in $\pi_q$ and the rank of documents starts from 0. Use $r_q^i$ and $\hat r_q^i$ to replace $r_q(x_i)$ and $\hat r_q(x_i)$ for simplicity. We have on $\pi_q$: 
\begin{align}
\label{eq:APR-loss}
    ARP
    =& \frac{1}{n}\sum_{i=1}^n rank(x_i|\pi_q)\cdot r_q^i\\\nonumber
    =& \frac{1}{2n}\sum_{i=1}^n\sum_{j=1}^n(r_q^i\mathbb I_{\hat r_q^i<\hat r_q^j}+r_q^j\mathbb I_{\hat r_q^j<\hat r_q^i})\\\nonumber
    %=& \frac{1}{n}\sum_{i=1}^n\Big(\sum_{j:r_q^j<r_q^i}r_q^i\mathbb I_{\hat r_q^i<\hat r_q^j}+r_q^j\mathbb I_{\hat r_q^j<\hat r_q^i}\Big)+\frac{1}{2n}\sum_{i=1}^n\sum_{j:r_q^i=r_q^j}r_q^j\\\nonumber
    =&\frac{1}{n}\sum_{i=1}^n\Big(\sum_{j:r_q^j<r_q^i}r_q^i\mathbb I_{\hat r_q^i<\hat r_q^j}+r_q^j\mathbb I_{\hat r_q^j<\hat r_q^i}\Big)+C_1\\\nonumber
    =&\frac{1}{n}\sum_{i=1}^n\sum_{j:r_q^j<r_q^i}|r_q^i-r_q^j|\mathbb I_{\hat r_q^i<\hat r_q^j}+C_1+C_2\\\nonumber
    (*)\leq&\frac{1}{n}\sum_{i=1}^n\sum_{j:r_q^j<r_q^i}|r_q^i-r_q^j|\log_2\big(1+e^{-\sigma(\hat r_q^i-\hat r_q^j)}\big)+C_1+C_2\\\nonumber
    %=&\frac{1}{n}\sum_{i,j:r_q^i>r_q^j}|r_q^i-r_q^j|\log_2\big(1+e^{-\sigma(\hat r_q^i-\hat r_q^j)}\big)+C_1+C_2
\end{align}
where $C_1=\frac{1}{2n}\sum_{i=1}^n\sum_{j:r_q^i=r_q^j}r_q^j$ and $C_2=\frac{1}{n}\sum_{i=1}^n\sum_{j:r_q^j<r_q^i}r_q^j$ ($C_2=0$ in binary case) are constants. As shown in step $*$, we should only impose pairwise loss to bound the comparison result indicator $\mathbb I_{\hat r_q^i<\hat r_q^j}$ on document pairs with different labels for optimizing the metric (relevant-irrelevant pairs in this binary case). Comparisons from pairs with the same label form a constant $C_1$ that does not contribute to the optimization. 

To be more specific, in $C_1$, a pair of documents with the same label $r$ count $r\mathbb{I}_{\hat r_q^i < \hat r_q^j} + r\mathbb{I}_{\hat r_q^j < \hat r_q^i} = r$ in the metric, which is a constant. However, if we introduce pairwise loss to bound each term, we are forcing the two predicted relevance values to be the same. Using pairwise logistic loss as an example, the loss $r\cdot\big[\log(1+\exp(-(\hat{r}_q^i - \hat{r}_q^j))) + \log(1+\exp(-(\hat{r}_q^j - \hat{r}_q^i)))\big]$ is minimized when $\hat{r}_q^i = \hat{r}_q^j$. In other words, the loss on a pair of documents with the same label impose unnecessary constraints that distort ranking metric optimization.  

The above analysis also generally applies to other ranking metrics like NDCG \cite{Wang2018Lambdaloss}. It %sets the foundation for optimizing ranking metrics with pairwise comparisons, which 
naturally generalizes to the unbiased LTR setting that uses implicit feedback for optimization. Next we will study the consequence of the pairwise loss in the IPS framework for unbiased learning to rank. 

\subsection{IPS for Practical Optimizations}
\label{sec:pairunbiasLTR}
Let us now focus on optimizing ranking metrics with IPS on implicit feedback. Consider a general pairwise loss $\delta(x_i,x_j|\pi_q)$ defined on two different documents $x_i$ and $x_j$ in $\pi_q$, which indicates how likely $x_i$ is more relevant than $x_j$. Following the IPS estimator in Eq~\eqref{eq:IPS}, the individual contribution of a relevant document $x_i$ to the ranking metric is upper bounded by the total pairwise loss of comparing $x_i$ to each other document in $\pi_q$:
\begin{equation}
\label{eq:bound}
    \Delta(x_i|\pi_q) \leq \sum_{x_j\in\pi_q\wedge x_j\neq x_i} \delta(x_i,x_j|\pi_q)
\end{equation}
where we assume minimizing the loss will optimize the metric. %Note that we can always flip the sign of $\Delta(x_i|\pi_q)$ accordingly, so that an upper bound is needed to optimize the ranking metric. 

In click data where only the relevant and observed documents are indicated by clicks, the local loss on $q$ can be derived from Eq~\eqref{eq:IPS} with pairwise loss for optimizing the ranking metric. There are currently two strategies for imposing the pairwise loss. The first one is to compare each clicked document to \emph{all} other documents as in Propensity SVM-Rank \cite{joachims2017ips}:
\begin{align}
\label{eq:click-all}
    l_{IPS}^{SVM}(\pi_q|q,\tilde\pi_q,o_q) = \mathop{\sum_{x_i:c_q(x_i)=1}}\frac{\sum_{x_j\in\pi_q\wedge x_j\neq x_i}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
% can contribute to the optimization of the ranking metric. 
In expectation, the above SVM-Rank based IPS estimator contains loss on all relevant-relevant pairs. 
%, because it compares a clicked document against all documents in $\pi_q$. 
However, as we discussed in Section \ref{sec:metric-optimization}, the pairwise loss should only be imposed on relevant-irrelevant document pairs for effective optimization. 

%Because the observed irrelevant labels are mixed with the unobserved labels (both unclicked), there is no irrelevance labels given. In the second strategy, unclicked documents are typically adopted as negative examples to compare to each clicked document to remove explicit comparisons of relevant-relevant pairs 
To avoid explicitly comparing two clicked documents, the second strategy restricts the loss on comparisons between clicked and unclicked ones \cite{rendle2009bpr,hu2019unbiasedlambda}:
\begin{align}
\label{eq:click-unclick}
    l_{IPS}(\pi_q|q,\tilde\pi_q,o_q) = \mathop{\sum_{x_i:c_q(x_i)=1}}\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
But as relevant and unobserved documents are also unclicked, this still cannot fully address the problem of including losses on relevant-relevant pairs that have no contribution to the optimization: 
\begin{align}
\label{eq:IPS-expectation}
    &E_{o_q}[l_{IPS}(\pi_q|q,\tilde\pi_q,o_q)] \\\nonumber
    =& E_{o_q}\bigg[\mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge\; r_q(x_i)=1}\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\bigg] \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}E_{o_q}\bigg[\frac{o_q(x_i)\cdot\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\bigg] \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\frac{P(o_q(x_i)=1|\tilde\pi_q)\cdot\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)} \\\nonumber
    %=& \sum_{x_i:r_q(x_i)=1}\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q) \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\bigg(\sum_{x_j\in\pi_q:r_q(x_j)=0}+\mathop{\sum_{x_j:o_q(x_j)=0}}_{\wedge r_q(x_j) = 1 }\bigg)\delta(x_i,x_j|\pi_q)
\end{align}
In expectation, %the IPS estimator is from the pairwise loss on relevant documents and unclciked documents. 
besides the pairwise loss on relevant-irrelevant pairs that we expect, this strategy also includes pairs on relevant documents versus relevant but unobserved documents (the second sum in the bracket). The negative effect can also be perceived from an intuitive perspective: as the relevant but unobserved documents are mistakenly used as negative examples, it will degrade the new ranker's ability to recognize these missed relevant documents, making the ranker still unfavorably biased for them.
%from two perspectives, both theoretically and intuitively: 1) it introduces terms that do not contribute to the ranking metric, thus dilutes the true loss for promoting relevant documents against irrelevant one; 2) as the relevant but unobserved documents are mistakenly used as negative examples, it will degrade the new ranker's ability to recognize these missed relevant documents, making the ranker still biased for them. 
\vspace{-0.5em}
\subsection{Empirical Effects}
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{pdf-figures/yahoo_pairwise_effect.pdf}
    \includegraphics[width=0.45\linewidth]{pdf-figures/web10k_pairwise_effect.pdf}
    \caption{The empirical performance applying IPS with pairwise loss. We compare the results of including pairwise loss on each clicked document and (1) all other documents; (2) unclicked documents; (3) only irrelevant documents.}
    \label{fig:effect}
\end{figure}
In order to verify our theoretical analysis, in Figure \ref{fig:effect}, we demonstrate the empirical influences of including relevant-relevant pairwise loss in LTR model training with clicks. Specifically, we synthesize clicks on the Yahoo and Web10K LTR datasets with the propensity model ($\eta=1$) described in Section \ref{sec:exp}. To better illustrate the effect, we adopt the noise-free setting and sampled 128,000 clicks. To learn new rankers from the clicks, we apply IPS on the pairwise logistic loss, and include pairs from different comparison strategies. The NDCG@10 results are reported on fully labeled test sets in the two benchmarks accordingly. As clearly shown, the performance of comparing clicked documents to only irrelevant achieves obvious improvements than the other two; including relevant-relevant document comparisons can hurt the ranker. 
%This experiment further verifies the adverse effects of counting losses on relevant-relevant pairs in optimization. 
Therefore, to eliminate such adverse effects for better LTR model learning, we should remove the relevant-relevant pairs by identifying the truly irrelevant documents in unclicked documents. In this way, we can ensure the induced loss to contribute to the ranking metric optimization. 

\section{Propensity Ratio Scoring for Unbiased Learning to Rank}
\label{sec:PRS-forunbiasedLTR}
We have shown that to effectively tackle unbiased LTR in practice, we need to avoid the relevant documents in unclicked documents when counting loss, and keep the total loss unbiased for all relevant documents. 
In this section, we first derive the solution of identifying truly irrelevant documents from unclicked ones, so that no relevant documents are used as negative examples. Then we develop a holistic treatment on using click data for optimizing the ranking metric with pairwise comparisons. %The goal is to remove the relevant documents from unclicked documents, and keep the total loss unbiased to the relevant documents.

\subsection{Propensity-weighted Negative Samples}
\label{sec:PNS}
The insight of identifying truly irrelvant documents in unclicked documents comes from the decomposition of click data in Figure \ref{fig:clickdata}. As mentioned, in a noise-free setting if the relevance label of a document is observed (the first column in Figure \ref{fig:clickdata}), click is equivalent to the relevance, i.e., $o_q(x_i)=1 \rightarrow [c_q(x_i)=r_q(x_i)]$. Then, if a document is observed and unclicked, it is irrelevant, i.e., $[o_q(x_i)=1 \wedge c_q(x_i)=0] \rightarrow r_q(x_i)=0$. In other words, if a document is unclicked but observed, it is irrelevant (i.e., the I\&O part in Figure \ref{fig:clickdata}). Therefore, the task of identifying truly irrelevant documents from unclicked ones is mapped to finding the observed documents in the unclicked ones. 

Note that for an unclicked document $x_j$, although we do not know the true observation $o_q(x_j)$, we can still estimate its observation propensity $o_q(x_j)\sim P(o_q(x_j)=1|\tilde\pi_q)$ \cite{Craswell2008clickpositionbias,wang2018pbe,Agarwal2019EPB}. 
By weighting the loss on each unclicked document with its observation propensity, in expectation we are able to restrict the loss on all unclicked documents to those that are unclicked but observed, which are truly irrelevant:
\begin{align}
\label{eq:PNS-expectation}
    &\sum_{x_j:c_q(x_j)=0}\Omega(x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q) \\\nonumber
    =&\; E_{o_q}[\mathop{\sum_{x_j:o_q(x_j)=1}}_{\wedge c_q(x_j)=0}\Omega(x_j|\pi_q)]\\\nonumber
    =&\; E_{o_q}[\mathop{\sum_{x_j:o_q(x_j)=1}}_{\wedge r_q(x_j)=0}\Omega(x_j|\pi_q)]\\\nonumber
\end{align}
where $\Omega(\cdot)$ represents any general loss on $x_j$, including the pairwise loss used in Section \ref{sec:pairunbiasLTR}. The last step is obtained by: $[o_q(x_j)=1 \wedge c_q(x_j)=0] \rightarrow r_q(x_j)=0$ (see Figure \ref{fig:clickdata}). We refer to this weighting on uncliked documents as the Propensity-weighted Negative Samples (PNS). 
%The effect of PNS is equivalent to sampling the unclicked documents with their propensities. 
This weighting scheme is also intuitive: if a document in the presented rank list is not clicked but very likely observed, we should have a high confidence that it is irrelevant. 
%For generality, PNS is able to recognize the truly negative examples from a set of examples without feedback, and can be generalized to other scenarios. For instance, in recommendation systems \cite{rendle2009bpr}, if an item is not interacted with a user, it is not necessarily disliked, but can also be unobserved. But high observation probability of an un-interacted item provides a strong signal of disliked. Also, in link prediction in social networks \cite{Liben2003link}, the distance between two nodes greatly influence the probability of being linked. No-link between two nodes does not mean they are not similar, while a short distance (high probability that they know each other) increase the chance of dissimilarity between them.

\subsection{Propensity Ratio Scoring}
\label{sec:PRS}
%We have proved that by weighting the unclicked documents with propensities, we can %identify the truly irrelevant documents (in expectation) and thus 
%avoid using relevant but unobserved documents as negative examples (in expectation). 
As the observation of documents are position-based and independent \cite{Craswell2008clickpositionbias,wang2018pbe}, weighting on clicked documents (with inverse propensities) and unclicked documents (with propensities) will not interfere with each other. Therefore, we can integrate them to reweight the pairwise loss inccured when comparing them:
\begin{align}
\label{eq:PRS}
    &l_{PRS}(\pi_q|q,\tilde\pi_q,o_q) \\\nonumber
    =& \mathop{\sum_{x_i:c_q(x_i)=1}}\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot\frac{P(o_q(x_j)=1|\tilde\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
which leads to a weight on each pairwise loss defined by the propensity ratio between the unclicked and clicked documents in it. We name this new weighting scheme Propensity Ratio Scoring, or PRS in short. In expectation, the PRS estimators can remove the relevant-relevant comparisons and compare each relevant document to \emph{only} irrelevant documents for metric optimization:
\begin{align}
\label{eq:PRS-expectation}
    &E_{o_q}\big[l_{PRS}(\pi_q|q,\tilde\pi_q,o_q)\big] \\\nonumber
    =& E_{o_q}\bigg[\mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge\; r_q(x_i)=1}\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\bigg] \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q) \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}E_{o_q}\big[\mathop{\sum_{x_j:r_q(x_j)=0}}_{\wedge o_q(x_j)=1}\delta(x_i,x_j|\pi_q)\big]
\end{align}
where the second step is the same as Eq~\eqref{eq:IPS-expectation}; and the third step is from Eq~\eqref{eq:PNS-expectation} by substituting $\Omega(x_j|\pi_q)$ with $\delta(x_i,x_j|\pi_q)$. This way, the total loss is purely obtained from valid relevant-irrelevant pairs that contribute to the ranking metric optimization. Notice that besides removing relevant documents from unclicked documents, Eq \eqref{eq:PRS-expectation} also
excludes the irrelevant and unobserved documents, i.e., the I\&U part in Figure \ref{fig:clickdata}. But because the ranking metrics are defined on relevant documents, we only need to correct the errors introduced by including relevant documents in negative examples, and keep the total loss unbiased to all relevant documents. As is demonstrated in the expectation, PRS can properly promote all the relevant documents against irrelevant documents without bias.
%avoids including relevant but unobserved documents as negative examples, and keeps the total loss unbiased to the relevant documents. 
%as the ranking metrics are defined on relevant documents. While no irrelevant document is promoted.

\subsubsection{Variability Analysis}
Besides the effect of removing relevant documents from negative examples, we show that by imposing a more careful use of the unclicked documents, the variability of the PRS estimator can be reduced comparing to the IPS estimator. Let us first rewrite the PRS estimator in Eq~\eqref{eq:PRS} as follows:
\begin{align*}
\label{eq:PRS-rewrite}
    &l_{PRS}(\pi_q|q,\tilde\pi_q,o_q) \\\nonumber
    %=& \mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge r_q(x_i)=1 }\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\\\nonumber
    =& \mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge r_q(x_i)=1 }\frac{1}{P(o_q(x_i)=1|\tilde\pi_q)}\cdot E_{o_q}\big[\mathop{\sum_{x_j:r_q(x_j)=0}}_{\wedge o_q(x_j)=1}\delta(x_i,x_j|\pi_q)\big]
\end{align*}
\begin{proposition}
    Let $N$ be the number of relevant documents retrieved for query $q$ and $P(o_q(x_i)=1|\tilde\pi_q)$ be the probability of independent Bernoulli events of observing each relevant document. According to Hoeffding's Inequality, for any given new ranking $\pi_q$, with probability of at least $1-\xi$, we have:
    \begin{equation*}
        \Big|l_{PRS}(\pi_q|q,\tilde\pi_q,o_q)-E_{o_q}\big[l_{PRS}(\pi_q|q,\tilde\pi_q,o_q)\big]\Big| \leq \frac{1}{N}\sqrt{\frac{log\frac{2}{\xi}}{2}\sum_{i=1}^{N}\rho_i^2}
    \end{equation*}
    where $\rho_i=\frac{1}{P(o_q(x_i)=1|\tilde\pi_q)}\cdot E_{o_q}\big[\sum_{x_j:r_q(x_j)=0 \wedge o_q(x_j)=1}\delta(x_i,x_j|\pi_q)\big]$ when $0<P(o_q(x_i)=1|\tilde\pi_q)<1$; otherwise, $\rho_i=0$.
\end{proposition}
The complete proof will be elaborated with details in a longer version of this paper. %But the key to prove this is to consider the loss on each relevant document as an independent Bernoulli variable in terms of observation. 
The above tail bound of the PRS estimator depicts its variability. Intuitively, this tail bound provides the range that the estimator can vary with a high probability; and a smaller range means a lower variability. Similarly, we can get the tail bound of the IPS estimator in Eq~\eqref{eq:click-unclick} as: 
\begin{equation*}
        \Big|l_{IPS}(\pi_q|q,\tilde\pi_q,o_q)-E_{o_q}\big[l_{IPS}(\pi_q|q,\tilde\pi_q,o_q)\big]\Big| \leq \frac{1}{N}\sqrt{\frac{log\frac{2}{\xi}}{2}\sum_{i=1}^{N}\tau_i^2}
    \end{equation*}
where $\tau_i=\frac{1}{P(o_q(x_i)=1|\tilde\pi_q)}\cdot \sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)$ if $0<P(o_q(x_i)=1|\tilde\pi_q)<1$; and $\tau_i=0$, otherwise. As the propensity of each unclicked document is smaller than 1, $0\leq\rho_i\leq\tau_i$ always holds, and thus the PRS estimator enjoys a reduced variability than the IPS estimator. This analysis predicts less variability and more stable performance of the PRS estimator compared to the IPS estimator.

\subsection{Incorporating Click Noise}
\label{sec:incorporatenoise}
We have assumed that the clicks are noise-free, i.e., a document is clicked if and only if it is observed and relevant: $c_q(x_i)=1\Leftrightarrow [o_q(x_i)=1\wedge r_q(x_i)=1]$. %In this setting, a clicked document must be relevant. 
However, in reality this could be violated: a user can possibly misjudge a relevant document, or mistakenly click on an irrelevant document. Specifically, we can introduce the noise in clicks in the same way as in \cite{joachims2017ips}:
\begin{align*}
    &P(c_q(x_i)=1|r_q(x_i)=1,o_q(x_i)=1) = \epsilon_+\\
    &P(c_q(x_i)=1|r_q(x_i)=0,o_q(x_i)=1) = \epsilon_-
\end{align*}
where $1\geq\epsilon_+>\epsilon_-\geq 0$ are the probability of clicking on a relevant or an irrelevant document, upon observation. %This assumption is mild and reasonable: if the clicking probability of an irrelevant document is even larger than a relevant document, it is impossible to learn a meaningful ranker. 
%From another perspective, this effect is equivalent to that the observed label of a document $\tilde r_q(x_i)$ is corrupted, i.e., $\tilde r_q(x_i)\neq r_q(x_i)$. 
Joachims et al. \cite{joachims2017ips} proved that such noise does not influence the optimization of IPS estimator under the metric ARP, which can be proved similarly under PRS. They key is to take expectation over the clicks upon observation. %However, such proofs can not generalize to other metrics or general loss used in practice. Fortunately, we found the PRS estimator is robust to the noise empirically, as PRS enjoys a lower variance and finer-grained use of the click data in general.  
We will further investigate the influence of noisy clicks empirically in Section \ref{sec:exp}. 
%similar to the IPS estimator \cite{joachims2017ips}, the optimization performed on the PRS estimator is robust to the noise. 


% \subsection{Propensity Estimation in Practice}
% \label{sec:propensity-estimate}
\begin{comment}
The application of the PRS estimator depends on the availability of the propensities, which is essential to unbiased LTR in practice. In particular, we focus on the position bias \cite{Craswell2008clickpositionbias,wang2018pbe}, i.e., the propensity of each document only depends on its position in the presented ranking. 
%There are several off-the-shelf methods proposed for estimating the position-based propensities. %, either from result randomization \cite{joachims2017ips}or directly estimate from click data \cite{wang2018pbe}. 
We describe the most representative estimation methods next. 

Consider the following position-based click propensity model:
\begin{equation*}
    P(c_q(x_i)=1|\tilde\pi_q) = P(e_q(x_i)=1|\tilde\pi_q,k)\cdot P\big(r_q(x_i)=1|e_q(x_i)=1,r_q(x_i)\big)
\end{equation*}
where $e_q(x_i)$ denotes whether the document is examined in $\tilde\pi_q$, and examination equals the observation of the relevance label: $e_q(x_i) = o_q(x_i)$. Thus the observation propensity estimation is equivalent to the position-based examination probability estimation. As this probability only depends on the position, we can use $p_k = P(e_q(x_i)=1|\tilde\pi_q,k)$ to denote the examination probability at position $k$.

A naive approach for estimating propensities is to randomize the presented results. In this way, the effect of the relevance label of a document could be eliminated, and thus the examination probability at each position equals to the click probability. However, such uniform randomization will drastically lower the search quality and result in undesired user experience. As we only need the relative ratio among the propensities across ranking positions, %a better way is to swap pairs at different positions. In \cite{joachims2017ips}, Joachims et al. randomly swap the top 1 document with documents at different positions. But 
a much smaller influence on the presented results could be achieved by swapping adjacent pairs, e.g., at position $k-1$ and $k$ \cite{wang2018pbe}. For each adjacent pair, we can get the relative observation ratio $\frac{p_k}{p_{k-1}}$, based on the number of clicks received on position $k-1$ and $k$. We can then obtain the relative ratio between any two positions:
\begin{equation*}
    \frac{p_k}{p_1} = \frac{p_2}{p_1}\cdot\frac{p_3}{p_2}\cdot\cdot\cdot\frac{p_k}{p_{k-1}}
\end{equation*}
%It has been empirically shown in \cite{wang2018pbe} that swapping adjacent pairs significantly reduce the negative effect from results randomization. 

Another line of approaches directly estimate propensities from clicks, by maximizing the likelihood of the assumed click models \cite{Fang2019InterventionHarvesting,agarwal2018consistent}. Wang et al. \cite{wang2018pbe} propose a regression-based EM algorithm to estimate propensities from regular clicks. Agarwal et al. \cite{Agarwal2019EPB} avoid the modeling of relevance labels and use an extremum estimator based on clicks logged from multiple different ranking functions. %But as propensity estimation is not the focus of this work, we leave it for our future exploration. 
\end{comment}

==> backups/old_method.tex <==
\section{The Issue of Inverse Propensity Scoring in Practice}
%2 issues from different perspectives: bias in the clicks on relevant documents && relevant documents in unclicked documents.
In this section, we first discuss the existing unbiased learning to rank framework based on Inverse Propensity Scoring (IPS). The key idea is to get an unbiased estimate of the ranking metric of interest from partially observed relevance labels in click data. We will start from its general formulation, and then prove its deficiency for unbiased learning to rank in practice. 
\subsection{Unbiased Learning to Rank}
\label{sec:unbiaLTR}
Without loss of generality, in LTR tasks we are given a set of i.i.d. queries $\bm{Q}$, where each query instance $q$ is sampled from an underlying distribution $q \sim P(q)$. Suppose we have a ranking system $S$, which generates a ranked list of documents $\pi_q$ retrieved for each query $q$. The order in $\pi_q$ is typically derived from the predicted \emph{relative} relevance values (or ranking scores) by $S$. Then the empirical risk $\mathcal{R}$ on $S$ is computed as:
\begin{equation*}
    \mathcal{R}(Q, S) = \frac{1}{|\bm Q|}\sum_{q\in\bm Q}R(\pi_q|q).
\end{equation*}
As the queries are independent and query-level analysis is not our focus in this work, we concentrate on the local risk from a single query $q$. Specifically, denote the relevance vector for all documents to query $q$ as $r_q$; and the ranked list $\pi_q$ is obtained by the predicted relevance values $\hat r_q$ by $S$. Let $x_i$ be a document in the ranked list, and $r_q(x_i)$ be the ground-truth relevance label of $x_i$ under query $q$. To simplify our discussion, assume the relevance label is binary, i.e., $r_q(x_i)\in \{0,1\}$. The goal of LTR is to optimize the ranking metric of our interest (e.g., ARP, NDCG, MAP, etc). Thus the local risk incurred on a query is defined on the ranking metric calculated on $\pi_q$. When the ranking metric is defined on relevant documents as in most cases \cite{joachims2017ips,ai2018DLA}, we can decompose the local risk as:
\begin{equation}
    R(\pi_q|q) = \sum_{x_i:r_q(x_i)=1}\Delta(x_i|\pi_q)
\end{equation}
where $\Delta(x_i|\pi_q)$ is the individual contribution from a relevant document $x_i$ to the ranking metric, e.g., the $rank$ of $x_i$ in ARP or the discounted gain of $x_i$ in NDCG. 

Unlike the full-information setting where the relevance labels of all documents in $\pi_q$ are known, $r_q$ is only partially observed in the implicit click feedback. 
In particular, the examination model \cite{richardson2007predicting} asserts that a user has to first examine a document to observe its relevance label before he/she decides to click it based on the relevance. Most relevance labels may remain unobserved. For example, given a presented ranking $\tilde\pi_q$, the relevance labels on the top-ranked documents are more likely to be observed than those on the lower-ranked positions, known as the position  bias \cite{wang2018pbe,Craswell2008clickpositionbias}. Following the counterfactual model introduced in \cite{joachims2017ips}, denote $o_q$ as a 0/1 vector indicating whether the relevance labels in $r_q$ are observed. For each element of $o_q$, the marginal probability $P(o_q(x_i)=1|\tilde\pi_q)$ of observing the relevance label $r_q(x_i)$ in $\tilde\pi_q$ is referred as the observation propensity of document $x_i$. Consider the deterministic noise-free setting in \cite{joachims2017ips}, %where examination of a document is equal to the observation of its relevance label. A
a document is clicked if and only if it is observed and relevant, i.e., $c_q(x_i)\Leftrightarrow o_q(x_i)\wedge r_q(x_i)$, while all other documents are recorded as unclicked. Note that an important property of click data is that only the positive feedback is logged, i.e., clicks. When a document is not clicked, it is unknown if it is irrelevant or not observed, as illustrated in Figure \ref{fig:clickdata}.
%This means even an irrelevance label is observed, it is not recorded in the implicit feedback. 
To be more explicit, we use another binary vector $c_q$ to denote whether each document is clicked under $q$. 

%Consider the deterministic noise-free setting in \cite{joachims2017ips}, where examination of a document is equal to the observation of its relevance label. A document is clicked if and only if it is observed and relevant, i.e., $c_q(x_i)\Leftrightarrow o_q(x_i)\wedge r_q(x_i)$, while all other documents are recorded as unclicked. As shown in Figure \ref{fig:clickdata}, the click data can be decomposed based on each document's true relevance label and whether it is observed. The unclicked documents are composed of irrelevant documents (both observed or unobserved) as well as relevant but unobserved documents. %There is no negative feedback.
%i.e., when the a relevant document is observed, it is clicked,  In Figure \ref{fig:clickdata}, we decompose the click data based on each document's relevance and whether the relevance label is observed. As is illustrated, the unclicked documents is composed with irrelevant documents (both observed or unobserved) as well as relevant but unobserved documents. There is no explicit negative feedback.  Specifically, we use another 0/1 vector $c_q$ to denote whether each document is clicked. 

Under this setting, given the clicks in a logged ranking $\tilde\pi_q$, we can get an unbiased estimate of $R(\pi_q|q)$ for any new ranking $\pi_q$ with the IPS estimator \cite{Imbens2015causal,Paul1983central}:
\begin{align}
\label{eq:IPS}
    R_{IPS}(\pi_q|q,\tilde\pi_q,o_q) &= \sum_{x_i:c_q(x_i)=1}\frac{\Delta(x_i|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)} \\\nonumber
    &= \mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge\; r_q(x_i)=1}\frac{\Delta(x_i|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
It has been proved that $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ provides an unbiased estimate of $R(\pi_q|q)$ for any new ranking $\pi_q$: $E_{o_q}[R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)]\\=R(\pi_q|q)$ \cite{joachims2017ips}. Thus optimizing $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ will lead to the same ranker as from $R(\pi_q|q)$, in terms of expectation. 

\subsection{Ranking Metrics Optimization}
Note that $R(\pi_q|q)$ and $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ are discrete metrics on relevant documents in a pointwise sense. They are not directly optimizable even with fully labeled relevance judgements \cite{Christopher2007nonsmooth}. In order to practically optimize the ranking metrics, we need to first calculate the metric on a ranking $\pi_q$ and formulate the optimizable loss with continuous approximations.

%$R(\pi_q|q)$ and $R_{IPS}(\pi_q|q,\tilde\pi_q,o_q)$ are discrete metrics on relevant documents. They are not directly optimizable even with fully labeled relevance judgements \cite{Christopher2007nonsmooth}. In order to practically optimize the ranking metrics, we need to first calculate the metric on a ranking $\pi_q$ and reformulate the risk with continuous approximations.

Firstly, the individual contribution $\Delta(x_i|\pi_q)$ of a relevant document has to be obtained from its comparisons to other documents in the ranking list $\pi_q$, as the ranking position of $x_i$ in $r_q$ depends on how many other documents are predicted to be more relevant than $x_i$ by $S$. As is shown in \cite{Wang2018Lambdaloss}, this could be realized via pairwise comparisons for a set of general ranking metrics. %This at least needs to be achieved via pairwise comparisons to all other documents in the list.
For instance, when getting the $rank$ of a relevant document $x_i$ in the ranked list $\pi_q$, we need to compare the predicted relevance between $\hat r_q(x_i)$ to each other document's $\hat r_q(x_j)$ in $\pi_q$. 
%Do we need to specify this with equations?
One important property that Wang et al. \cite{Wang2018Lambdaloss} %propose a general framework for optimizing ranking metrics with pairwise comparisons, which unifies the theoretical foundations of popularly used pairwise ranking algorithms.  being 
has proved is that the comparisons between two documents of the same label will form a constant term in the ranking metric, agnostic to their positions or predicted relevance values. Hence, \emph{only} the comparisons between documents of different labels affect the ranking metrics and therefore can contribute to the optimization. 

Secondly, although we can obtain the ranking metrics on $\pi_q$ from pairwise comparisons, the resulting metrics are still discrete. Thus continuous approximations that bound the ranking metrics are needed for practical optimization. For example, logistic loss \cite{Arias2008logistic} or hinge loss \cite{Joachims2002OSE} are typical approximations for pairwise comparisons that bound the ranking metric of our interest. Equivalently, one can also introduce the approximations on the gradient of the ranking metric from pairwise comparisons, such as the lambda loss in LambdaRank \cite{burges2010from} (see Section 5 in \cite{Wang2018Lambdaloss}). Based on the first point, the pairwise loss should be imposed \emph{only} on the document pairs with different labels, which can really contribute to the ranking metric optimization. Imposing loss on document pairs with the same label will introduce extra irreducible terms in the final loss that distort the optimization and lead to sub-optimal results. 

To theoretically illustrate our analysis above, we take the optimization of Average Relevance Position used in \cite{joachims2017ips} as an example. Assume there are $n$ documents in $\pi_q$ and the rank of documents starts from 0. To simplify the notations, we use $r_q^i$ and $\hat r_q^i$ to replace $r_q(x_i)$ and $\hat r_q(x_i)$ respectively. Then we have: 
\begin{align}
\label{eq:APR-loss}
    ARP
    =& \frac{1}{n}\sum_{i=1}^n rank(x_i|\pi_q)\cdot r_q^i\\\nonumber
    =& \frac{1}{2n}\sum_{i=1}^n\sum_{j=1}^n(r_q^i\mathbb I_{\hat r_q^i<\hat r_q^j}+r_q^j\mathbb I_{\hat r_q^j<\hat r_q^i})\\\nonumber
    =& \frac{1}{n}\sum_{i=1}^n\Big(\sum_{j:r_q^j<r_q^i}r_q^i\mathbb I_{\hat r_q^i<\hat r_q^j}+r_q^j\mathbb I_{\hat r_q^j<\hat r_q^i}\Big)+\frac{1}{2n}\sum_{i=1}^n\sum_{j:r_q^i=r_q^j}r_q^j\\\nonumber
    =&\frac{1}{n}\sum_{i=1}^n\Big(\sum_{j:r_q^j<r_q^i}r_q^i\mathbb I_{\hat r_q^i<\hat r_q^j}+r_q^j\mathbb I_{\hat r_q^j<\hat r_q^i}\Big)+C_1\\\nonumber
    =&\frac{1}{n}\sum_{i=1}^n\sum_{j:r_q^j<r_q^i}|r_q^i-r_q^j|\mathbb I_{\hat r_q^i<\hat r_q^j}+C_1+C_2\\\nonumber
    (*)\leq&\frac{1}{n}\sum_{i=1}^n\sum_{j:r_q^j<r_q^i}|r_q^i-r_q^j|\log_2\big(1+e^{-\sigma(\hat r_q^i-\hat r_q^j)}\big)+C_1+C_2\\\nonumber
    =&\frac{1}{n}\sum_{i,j:r_q^i>r_q^j}|r_q^i-r_q^j|\log_2\big(1+e^{-\sigma(\hat r_q^i-\hat r_q^j)}\big)+C_1+C_2
\end{align}
where $C_1=\frac{1}{2n}\sum_{i=1}^n\sum_{j:r_q^i=r_q^j}r_q^j$ and $C_2=\frac{1}{n}\sum_{i=1}^n\sum_{j:r_q^j<r_q^i}r_q^j$ ($C_2=0$ in binary case) are constants. As shown in step $*$, we should only add pairwise loss to bound the comparison result indicator $\mathbb I_{\hat r_q^i<\hat r_q^j}$ on document pairs with different labels for optimizing the metric (relevant-irrelevant pairs in this binary case). Comparisons from pairs with the same label form a constant $C_1$ that does not contribute to the optimization. 

To be more specific, in $C_1$, a pair of documents with the same label $r$ count $r\mathbb{I}_{\hat r_q^i < \hat r_q^j} + r\mathbb{I}_{\hat r_q^j < \hat r_q^i} = r$ in the metric. It is a constant regardless of their predicted relevance values. However, if we introduce pairwise loss to bound each term, we are forcing the two predicted relevance values to be the same. Using pairwise logistic loss as an example, the loss $r\cdot\big[\log(1+exp(-(\hat{r}_q^i - \hat{r}_q^j))) + \log(1+e(-(\hat{r}_q^j - \hat{r}_q^i)))\big]$ is minimized when $\hat{r}_q^i = \hat{r}_q^j$. In other words, the loss on a pair of documents with the same label impose unnecessary constraints to the ranking metric optimization.  % and metric for LambdaRank, respectively.

The above analysis also generally applies to other ranking metrics (see Section 5 in \cite{Wang2018Lambdaloss} for optimizing other metrics such as NDCG). It sets the foundation for optimizing ranking metrics with pairwise comparisons, which naturally generalize to the unbiased LTR setting that uses implicit feedback for optimization. Next we will investigate the consequence of the pairwise loss in the unbiased learning to rank framework. 

\subsection{Formulation using Pairwise Comparisons}
\label{sec:pairunbiasLTR}
Let us now focus on optimizing ranking metrics with implicit feedback. Consider a general pairwise loss $\delta(x_i,x_j|\pi_q)$ defined on two different documents $x_i$ and $x_j$ in $\pi_q$, which indicates how likely $x_i$ is more relevant than $x_j$. Following the IPS estimator in Eq~\eqref{eq:IPS}, the individual contribution of a relevant document $x_i$ to the ranking metric is upper bounded by the total pairwise loss of comparing $x_i$ to each other document in $\pi_q$:
\begin{equation}
\label{eq:bound}
    \Delta(x_i|\pi_q) \leq \sum_{x_j\in\pi_q\wedge x_j\neq x_i} \delta(x_i,x_j|\pi_q)
\end{equation}
where we assume minimizing the loss will optimize the metric. Note that we can always flip the sign of $\Delta(x_i|\pi_q)$ accordingly, so that an upper bound is needed to optimize the ranking metric. 

In click data where only the relevant and observed documents are indicated by clicks, the local loss on $q$ can be derived from Eq~\eqref{eq:IPS} with pairwise loss for optimizing the ranking metric. There are currently two strategies for imposing the pairwise loss. The first one is to compare each clicked document to \emph{all} other documents as in Propensity SVM-Rank \cite{joachims2017ips}:
\begin{align}
\label{eq:click-all}
    l_{IPS}^{SVM}(\pi_q|q,\tilde\pi_q,o_q) = \mathop{\sum_{x_i:c_q(x_i)=1}}\frac{\sum_{x_j\in\pi_q\wedge x_j\neq x_i}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
% can contribute to the optimization of the ranking metric. 
In expectation, the above SVM-Rank based IPS estimator contains loss on all relevant-relevant pairs. 
%, because it compares a clicked document against all documents in $\pi_q$. 
However, as we discussed in Section \ref{sec:unbiaLTR}, the pairwise loss should only be imposed on relevant-irrelevant document pairs for effective optimization. 

%Because the observed irrelevant labels are mixed with the unobserved labels (both unclicked), there is no irrelevance labels given. In the second strategy, unclicked documents are typically adopted as negative examples to compare to each clicked document to remove explicit comparisons of relevant-relevant pairs 
To avoid explicitly comparing two clicked documents, the second strategy restricts the loss on comparisons between clicked and unclicked ones \cite{rendle2009bpr,hu2019unbiasedlambda}:
\begin{align}
\label{eq:click-unclick}
    l_{IPS}(\pi_q|q,\tilde\pi_q,o_q) = \mathop{\sum_{x_i:c_q(x_i)=1}}\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
But as relevant and unobserved documents are also in the unclicked part, this strategy stll cannot fully address the problem of including losses on relevant-relevant pairs that have no contribution to the optimization: 
\begin{align}
\label{eq:IPS-expectation}
    &E_{o_q}[l_{IPS}(\pi_q|q,\tilde\pi_q,o_q)] \\\nonumber
    =& E_{o_q}\bigg[\mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge\; r_q(x_i)=1}\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\bigg] \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}E_{o_q}\bigg[\frac{o_q(x_i)\cdot\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\bigg] \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\frac{P(o_q(x_i)=1|\tilde\pi_q)\cdot\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)} \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q) \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\bigg(\sum_{x_j\in\pi_q:r_q(x_j)=0}+\mathop{\sum_{x_j:o_q(x_j)=0}}_{\wedge r_q(x_j) = 1 }\bigg)\delta(x_i,x_j|\pi_q)
\end{align}
In expectation, %the IPS estimator is from the pairwise loss on relevant documents and unclciked documents. 
besides the pairwise loss on relevant-irrelevant pairs that we expect, this strategy also includes pairs on relevant documents versus relevant but unobserved documents. The negative effect can also be perceived from a intuitive perspective: as the relevant but unobserved documents are mistakenly used as negative examples, it will degrade the new ranker's ability to recognize these missed relevant documents, making the ranker still biased for them.
%from two perspectives, both theoretically and intuitively: 1) it introduces terms that do not contribute to the ranking metric, thus dilutes the true loss for promoting relevant documents against irrelevant one; 2) as the relevant but unobserved documents are mistakenly used as negative examples, it will degrade the new ranker's ability to recognize these missed relevant documents, making the ranker still biased for them. 
\vspace{-0.5em}
\subsection{Empirical Effects}
\begin{figure}
    \centering
    \includegraphics[width=0.47\linewidth]{pdf-figures/yahoo_pairwise_effect.pdf}
    \includegraphics[width=0.47\linewidth]{pdf-figures/web10k_pairwise_effect.pdf}
    \caption{The empirical performance applying IPS with pairwise loss. We compare the results of including pairwise loss on each clicked document and (1) all other documents; (2) unclicked documents; (3) only irrelevant documents.}
    \label{fig:effect}
\end{figure}
In order to verify our theoretical analysis, in Figure \ref{fig:effect}, we demonstrate the empirical results of including relevant-relevant pairwise loss in LTR model training. Specifically, we synthesize clicks on the Yahoo and Web10K LTR datasets with the propensity model ($\eta=1$) described in Section \ref{sec:exp}. To better illustrate the effect, we adopt the noise-free setting and sampled 128,000 clicks. To learn new rankers from the clicks, we apply IPS on the pairwise logistic loss, and include pairs from different comparison strategies. The NDCG@10 results are reported on fully labeled test sets in the two benchmarks accordingly. As clearly shown, the performance of comparing clicked documents to only irrelevant achieves obvious improvements than the other two; including relevant-relevant document comparisons can hurt the ranker. 
%This experiment further verifies the adverse effects of counting losses on relevant-relevant pairs in optimization. 
Therefore, to eliminate such adverse effects for better LTR model learning, we should remove the relevant-relevant pairs by identifying the truly irrelevant documents in unclicked documents. In this way, we can ensure the induced loss to contribute to the ranking metric optimization. 

\section{Propensity Ratio Scoring for Unbiased Learning to Rank}
\label{sec:PRS-forunbiasedLTR}
Up to this point, we have shown that to effectively apply unbiased LTR in practice, %although the bias of using clicks to represent relevant documents can be addressed with IPS, 
we need to remove the relevant documents in unclicked documents when counting loss, and keep the total loss unbiased on the relevant documents. %As is indicated in Eq~\ref{eq:IPS}, we can keep the IPS on clicked documents to get an unbiased estimate of the ranking metric defined on relevant documents. 
In this section, we first focus on deriving the solution of identifying truly irrelevant documents from unclicked ones, so that no relevant documents are used as negative examples. Then we develop a holistic treatment on using click data for optimizing the ranking metric with pairwise comparisons. %The goal is to remove the relevant documents from unclicked documents, and keep the total loss unbiased to the relevant documents.

\subsection{Propensity-weighted Negative Samples}
\label{sec:PNS}
Our insight of identifying truly irrelvant documents in unclicked documents comes from the decomposition of click data in Figure \ref{fig:clickdata}. As mentioned before, in a noise-free setting if the relevance label of a document is observed (the first column in Figure \ref{fig:clickdata}), click is equivalent to the relevance, i.e., $o_q(x_i)=1 \rightarrow [c_q(x_i)=r_q(x_i)]$. Then, if a document is observed and unclicked, it is irrelevant, i.e., $[o_q(x_i)=1 \wedge c_q(x_i)=0] \rightarrow r_q(x_i)=0$. In other words, if a document is unclicked but observed, it is irrelevant (i.e., the I\&O part in Figure \ref{fig:clickdata}). Therefore, the task of identifying truly irrelevant documents from unclicked ones is mapped to finding the observed documents in the unclicked ones. 

Note that for an unclicked document $x_j$, although we do not know the true observation $o_q(x_j)$, we can estimate its observation propensity $o_q(x_j)\sim P(o_q(x_j)=1|\tilde\pi_q)$ (see Section \ref{sec:propensity-estimate}). %For example, when the observation propensity only depends on the position of each document in the ranked list as mostly studied, we can estimate the probability at each position through randomization. 
By weighting the loss on each unclicked document with its observation propensity, in expectation we can restrict the loss on all unclicked documents to those that are unclicked but also observed, which are truly irrelevant:
\begin{align}
\label{eq:PNS-expectation}
    &\sum_{x_j:c_q(x_j)=0}\Omega(x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q) \\\nonumber
    =&\; E_{o_q}[\sum_{x_j:c_q(x_j)=0}\Omega(x_j|\pi_q)\cdot o_q(x_j)]\\\nonumber
    =&\; E_{o_q}[\mathop{\sum_{x_j:c_q(x_j)=0}}_{\wedge o_q(x_j)=1}\Omega(x_j|\pi_q)]\\\nonumber
    =&\; E_{o_q}[\mathop{\sum_{x_j:r_q(x_j)=0}}_{\wedge o_q(x_j)=1}\Omega(x_j|\pi_q)]\\\nonumber
\end{align}
where $\Omega(\cdot)$ represents any kind of loss on $x_j$, including the pairwise loss used in Section \ref{sec:pairunbiasLTR}. The last step is obtained by: $[o_q(x_j)=1 \wedge c_q(x_j)=0] \rightarrow r_q(x_j)=0$ (see Figure \ref{fig:clickdata}). We refer to this weighting on uncliked documents as the Propensity-weighted Negative Samples (PNS). 
%The effect of PNS is equivalent to sampling the unclicked documents with their propensities. 
The new weighting scheme is also intuitive: if a document in the presented rank list is not clicked but very likely observed, we should have a high confidence that it is irrelevant. 
%For generality, PNS is able to recognize the truly negative examples from a set of examples without feedback, and can be generalized to other scenarios. For instance, in recommendation systems \cite{rendle2009bpr}, if an item is not interacted with a user, it is not necessarily disliked, but can also be unobserved. But high observation probability of an un-interacted item provides a strong signal of disliked. Also, in link prediction in social networks \cite{Liben2003link}, the distance between two nodes greatly influence the probability of being linked. No-link between two nodes does not mean they are not similar, while a short distance (high probability that they know each other) increase the chance of dissimilarity between them.

\subsection{Propensity Ratio Scoring}
\label{sec:PRS}
We have proved that PNS identifies the truly irrelevant documents (in expectation) and thus avoids using relevant but unobserved documents as negative examples. As the examination of documents are only position-based and independent (see Section \ref{sec:propensity-estimate}), PNS will not interfere with IPS in weighting clicked and unclicked documents. Therefore, we can apply IPS to the clicked document and PNS to the unclicked document to reweight the pairwise loss inccured when comparing them:
\begin{align}
\label{eq:PRS}
    &l_{PRS}(\pi_q|q,\tilde\pi_q,o_q) \\\nonumber
    =& \mathop{\sum_{x_i:c_q(x_i)=1}}\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot\frac{P(o_q(x_j)=1|\tilde\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}
\end{align}
which leads to a weight on each pairwise loss defined by the propensity ratio between the unclicked and clicked documents in it. We name this new weighting scheme Propensity Ratio Scoring, or PRS in short. In expectation, the PRS estimator can remove the relevant-relevant comparisons and compare each relevant document to \emph{only} irrelevant documents for metric optimization:
\begin{align}
\label{eq:PRS-expectation}
    &E_{o_q}\big[l_{PRS}(\pi_q|q,\tilde\pi_q,o_q)\big] \\\nonumber
    =& E_{o_q}\bigg[\mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge\; r_q(x_i)=1}\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\bigg] \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q) \\\nonumber
    =& \sum_{x_i:r_q(x_i)=1}E_{o_q}\big[\mathop{\sum_{x_j:r_q(x_j)=0}}_{\wedge o_q(x_j)=1}\delta(x_i,x_j|\pi_q)\big]
\end{align}
where the second step is the same as Eq~\eqref{eq:IPS-expectation}; and the third step is from Eq~\eqref{eq:PNS-expectation} by substituting $\Omega(x_j|\pi_q)$ with $\delta(x_i,x_j|\pi_q)$. This way, we can eliminate the pairwise loss on relevant-relevant pairs, and thus the total loss is purely obtained from valid pairs that contribute to the ranking metric optimization. One may notice that besides removing relevant documents from unclicked documents, Eq \eqref{eq:PRS-expectation} also
excludes the irrelevant and unobserved documents, i.e., the I\&U part in Figure \ref{fig:clickdata}. But because the ranking metrics are defined on relevant documents, we only need to correct the errors introduced by including relevant documents in negative examples, and keep the total loss unbiased to the relevant documents. As is demonstrated in the expectation, PRS can properly promote all the relevant documents against irrelevant documents without bias.
%avoids including relevant but unobserved documents as negative examples, and keeps the total loss unbiased to the relevant documents. 
%as the ranking metrics are defined on relevant documents. While no irrelevant document is promoted.

\subsubsection{Variability Analysis}
Besides the effect of removing relevant documents from negative examples, we show that by imposing a more careful use of the unclicked documents, the variability of the PRS estimator can be substantially reduced comparing to the IPS estimator. Let us first rewrite the PRS estimator in Eq~\eqref{eq:PRS} as follows:
\begin{align*}
\label{eq:PRS-rewrite}
    &l_{PRS}(\pi_q|q,\tilde\pi_q,o_q) \\\nonumber
    %=& \mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge r_q(x_i)=1 }\frac{\sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)\cdot P(o_q(x_j)=1|\tilde\pi_q)}{P(o_q(x_i)=1|\tilde\pi_q)}\\\nonumber
    =& \mathop{\sum_{x_i:o_q(x_i)=1}}_{\wedge r_q(x_i)=1 }\frac{1}{P(o_q(x_i)=1|\tilde\pi_q)}\cdot E_{o_q}\big[\mathop{\sum_{x_j:r_q(x_j)=0}}_{\wedge o_q(x_j)=1}\delta(x_i,x_j|\pi_q)\big]
\end{align*}
\begin{proposition}
    Let $N$ be the number of relevant documents retrieved for query $q$ and $P(o_q(x_i)=1|\tilde\pi_q)$ be the probability of independent Bernoulli events of observing each relevant document. According to Hoeffding's Inequality, for any given new ranking $\pi_q$, with probability of at least $1-\xi$, we have:
    \begin{equation*}
        \Big|l_{PRS}(\pi_q|q,\tilde\pi_q,o_q)-E_{o_q}\big[l_{PRS}(\pi_q|q,\tilde\pi_q,o_q)\big]\Big| \leq \frac{1}{N}\sqrt{\frac{log\frac{2}{\xi}}{2}\sum_{i=1}^{N}\rho_i^2}
    \end{equation*}
    where $\rho_i=\frac{1}{P(o_q(x_i)=1|\tilde\pi_q)}\cdot E_{o_q}\big[\sum_{x_j:r_q(x_j)=0 \wedge o_q(x_j)=1}\delta(x_i,x_j|\pi_q)\big]$ when $0<P(o_q(x_i)=1|\tilde\pi_q)<1$; otherwise, $\rho_i=0$.
\end{proposition}
The complete proof will be elaborated with details in a longer version of this paper. %But the key to prove this is to consider the loss on each relevant document as an independent Bernoulli variable in terms of observation. 
The above tail bound of the PRS estimator depicts its variability. Intuitively, this tail bound provides the range that the estimator can vary with a high probability; and a smaller range means a lower variability. Similarly, we can get the tail bound of the IPS estimator in Eq~\eqref{eq:click-unclick} as: 
\begin{equation*}
        \Big|l_{IPS}(\pi_q|q,\tilde\pi_q,o_q)-E_{o_q}\big[l_{IPS}(\pi_q|q,\tilde\pi_q,o_q)\big]\Big| \leq \frac{1}{N}\sqrt{\frac{log\frac{2}{\xi}}{2}\sum_{i=1}^{N}\tau_i^2}
    \end{equation*}
where $\tau_i=\frac{1}{P(o_q(x_i)=1|\tilde\pi_q)}\cdot \sum_{x_j:c_q(x_j)=0}\delta(x_i,x_j|\pi_q)$ if $0<P(o_q(x_i)=1|\tilde\pi_q)<1$; and $\tau_i=0$, otherwise. As the propensity of each unclicked document is smaller than 1, $0\leq\rho_i\leq\tau_i$ always holds, and thus the PRS estimator enjoys a reduced variability than the IPS estimator. This analysis predicts less variability and more stable performance of the PRS estimator compared to the IPS estimator.

\subsection{Incorporating Click Noise}
\label{sec:incorporatenoise}
We have assumed that the clicks are noise-free, i.e., a document is clicked if and only if it is observed and relevant: $c_q(x_i)=1\Leftrightarrow [o_q(x_i)=1\wedge r_q(x_i)=1]$. %In this setting, a clicked document must be relevant. 
However, in reality this could be violated: a user can possibly misjudge a relevant document, or mistakenly click on an irrelevant document. Specifically, we can introduce the noise in clicks in the same way as \cite{joachims2017ips}:
\begin{align*}
    &P(c_q(x_i)=1|r_q(x_i)=1,o_q(x_i)=1) = \epsilon_+\\
    &P(c_q(x_i)=1|r_q(x_i)=0,o_q(x_i)=1) = \epsilon_-
\end{align*}
where $1\geq\epsilon_+>\epsilon_-\geq 0$ are the probability of clicking on a relevant or an irrelevant document, upon observation. %This assumption is mild and reasonable: if the clicking probability of an irrelevant document is even larger than a relevant document, it is impossible to learn a meaningful ranker. 
%From another perspective, this effect is equivalent to that the observed label of a document $\tilde r_q(x_i)$ is corrupted, i.e., $\tilde r_q(x_i)\neq r_q(x_i)$. 
Joachims et al. \cite{joachims2017ips} proved that such noise does not influence the optimization of IPS estimator under the metric ARP, which can be proved similarly under PRS. They key is to take expectation over the clicks upon observation. %However, such proofs can not generalize to other metrics or general loss used in practice. Fortunately, we found the PRS estimator is robust to the noise empirically, as PRS enjoys a lower variance and finer-grained use of the click data in general.  
We will further investigate the influence of noisy clicks empirically in Section \ref{sec:exp}. 
%similar to the IPS estimator \cite{joachims2017ips}, the optimization performed on the PRS estimator is robust to the noise. 

\subsection{Propensity Estimation in Practice}
\label{sec:propensity-estimate}
The application of the PRS estimator depends on the availability of the propensities, which is essential to unbiased LTR in practice. In particular, we focus on the position bias \cite{Craswell2008clickpositionbias,wang2018pbe}, i.e., the propensity of each document only depends on its position in the presented ranking. 
%There are several off-the-shelf methods proposed for estimating the position-based propensities. %, either from result randomization \cite{joachims2017ips}or directly estimate from click data \cite{wang2018pbe}. 
We describe the most representative estimation methods next. 

Consider the following position-based click propensity model:
\begin{equation*}
    P(c_q(x_i)=1|\tilde\pi_q) = P(e_q(x_i)=1|\tilde\pi_q,k)\cdot P\big(r_q(x_i)=1|e_q(x_i)=1,r_q(x_i)\big)
\end{equation*}
where $e_q(x_i)$ denotes whether the document is examined in $\tilde\pi_q$, and examination equals the observation of the relevance label: $e_q(x_i) = o_q(x_i)$. Thus the observation propensity estimation is equivalent to the position-based examination probability estimation. As this probability only depends on the position, we can use $p_k = P(e_q(x_i)=1|\tilde\pi_q,k)$ to denote the examination probability at position $k$.

A naive approach for estimating propensities is to randomize the presented results. In this way, the effect of the relevance label of a document could be eliminated, and thus the examination probability at each position equals to the click probability. However, such uniform randomization will drastically lower the search quality and result in undesired user experience. As we only need the relative ratio among the propensities across ranking positions, %a better way is to swap pairs at different positions. In \cite{joachims2017ips}, Joachims et al. randomly swap the top 1 document with documents at different positions. But 
a much smaller influence on the presented results could be achieved by swapping adjacent pairs, e.g., at position $k-1$ and $k$ \cite{wang2018pbe}. For each adjacent pair, we can get the relative observation ratio $\frac{p_k}{p_{k-1}}$, based on the number of clicks received on position $k-1$ and $k$. We can then obtain the relative ratio between any two positions:
\begin{equation*}
    \frac{p_k}{p_1} = \frac{p_2}{p_1}\cdot\frac{p_3}{p_2}\cdot\cdot\cdot\frac{p_k}{p_{k-1}}
\end{equation*}
%It has been empirically shown in \cite{wang2018pbe} that swapping adjacent pairs significantly reduce the negative effect from results randomization. 

Another line of approaches directly estimate propensities from clicks, by maximizing the likelihood of the assumed click models \cite{Fang2019InterventionHarvesting,agarwal2018consistent}. Wang et al. \cite{wang2018pbe} propose a regression-based EM algorithm to estimate propensities from regular clicks. Agarwal et al. \cite{Agarwal2019EPB} avoid the modeling of relevance labels and use an extremum estimator based on clicks logged from multiple different ranking functions. %But as propensity estimation is not the focus of this work, we leave it for our future exploration. 


==> long-rel-work.tex <==
\section{Related Work}
% Using implicit feedback for ranking, exist the bias issue
% Click models and randomization to address the bias issue
% Unbiased learning to rank methods, IPS
% Recent progress in IPS based variants and propensity estimation
% Brief introduction of PRS.

% Click data has been a vital resource for LTR model training in modern retrieval systems. Compared to explicit relevance judgements, which are typically elicited from experts or crowdsourcing workers, click-based implicit feedback is easy to collect and substantially more timely \cite{Joachims2002OSE}. But the intrinsic bias, especially the position or presentation bias, limits its effective use \cite{Joachims2007Eval,yue2010beyondposition}. %In \cite{Joachims2017interpretclick}, Joachims et al. show via a user study that click data can reveal reasonably accurate relative relevance, as long as certain bias are taken into account, especially the presentation (or position) bias. 

Click data is a vital resource for LTR model training in modern retrieval systems. But the intrinsic bias, especially the position bias, limits its effective use \cite{Joachims2007Eval,yue2010beyondposition}. Various solutions have been proposed to address the bias issue for subsequent LTR training. For example, numerous click models \cite{chuklin2015click, Craswell2008clickpositionbias, Chapelle2009dynamicbayesian, Dupret2008UBM, Wang2013contentaware} are proposed to model the bias in users' result examination and click behaviors, so as to extract true relevance labels. %For example, the cascade model \cite{Craswell2008clickpositionbias} assumes that a user sequentially browse the ranking results from top to bottom, and will click on a document if it is relevant.
%Numerous click models \cite{Craswell2008clickpositionbias,Chapelle2009dynamicbayesian, Dupret2008UBM, Wang2013contentaware} have been developed under different assumptions about users' click decisions. 
But they require repeated observations for reliable relevance inference. %, and the objective is to maximize the likelihood rather than the ranking performance. 
Researchers also adopt randomization to eliminate bias \cite{Chapelle2012interleave,yue2009interactively,Swaminathan2015batchlearning} when collecting clicks. %As documents are randomly presented \cite{Swaminathan2015batchlearning} or swapped \cite{Raman2013LearningSocially} at different positions, user clicks collected in this way can reveal the true preferences and avoid the trouble of modeling user behaviors.
Though assumption free, randomization degrades the ranking quality during data collection and inevitably hurts user experience. %Both approaches first infer the unbiased relevance judgements from clicks and then apply LTR methods. 

To address these limitations, recent efforts focus on unbiased LTR directly from biased click data. %The main stem of solutions root in the techniques developed for observational studies in causal inference \cite{Imbens2015causal,Little1986statistical}. 
The key idea is to obtain an unbiased estimator of a ranking metric of interest by leveraging statistical patterns embedded in the logged click data. % For example, Wang et al. \cite{Wangselectionbias} apply inverse propensity scoring (IPS) to address the selection bias at the query level. 
Inverse propensity scoring (IPS) \cite{joachims2017ips} is a mainstream solution of this type, which reweighs observational implicit feedback for the debiasing purpose. 
%Despite the extensive use of IPS, it is shown that only when there is little bias and noise can IPS based methods outperform online methods \cite{Jagerman2019modelorintervene}. 
However, IPS is solely applicable to debias clicked documents, and its utility largely depend on whether most relevant documents can be revealed by the clicks. When there is increasing bias or noise, more relevant documents are buried in non-clicked documents, which IPS cannot handle. To make things even worse, IPS-based methods treat those non-clicked but relevant documents as negative samples for ranker training \cite{hu2019unbiasedlambda}. 
%IPS can no longer properly recognize and promote the relevant but unclicked documents, 
This directly leads to its poor performance in practice \cite{Jagerman2019modelorintervene}, and we theoretically prove the cause of this deficiency in this paper. % In contrast, we take a holistic treatment of click data in this work, and derive a well justified solution that accounts for the use of both clicks and non-clicks. 

There exists several realizations of the IPS framework for unbiased LTR \cite{wang2018pbe, ai2018DLA, hu2019unbiasedlambda}. Though based on different algorithms or model structures, they suffer from the same issues of IPS. Among them, Hu el al. \cite{hu2019unbiasedlambda} applied IPS to both clicked and non-clicked documents for debiasing. However, this solution ignores the fact that the bias issue in clicked and non-clicked documents are  \emph{asymmetric}, and simply assumes that unclick probability is proportional to the irrelevance probability to apply IPS. In contrast, we carefully analyze the bias issue 
rooted in non-clicked documents and derive a well justified solution that accounts for the use of both clicks and non-clicks. 

% take a holistic treatment of click data in this work, and derive a well justified solution that accounts for the use of both clicks and non-clicks. 

%Primary applications of unbiased LTR methods depend on the existence of propensities, which represent the observation bias in clicks. Propensities are usually estimated in a separate procedure and different estimation methods focusing on the position bias have emerged recently. Result randomization or swapping is one of the most basic ways for estimating the position bias \cite{joachims2017ips}. But there are also methods that directly estimate propensities from clicks. For example Wang et al. \cite{wang2018pbe} propose an EM algorithm to estimate propensities from logged clicks. Some other methods are proposed as well to improve the efficiency and accuracy of position bias estimation (see \cite{Fang2019InterventionHarvesting,Agarwal2019EPB,agarwal2018consistent}). There are also works that put forward the idea of jointly estimate the propensities and an unbiased ranker \cite{ai2018DLA, hu2019unbiasedlambda}. But they are all based on the IPS framework and adopt heuristics to some extents. %For instance, Hu el al. \cite{hu2019unbiasedlambda} assume that unclick probability is proportional to the irrelevance probability. 
%In this work, we inherit the existing methods for estimating the propensities and concentrate on the theoretical foundations for unbiased LTR. 



==> online_exp.tex <==
\section{Real-World Experiment}
To evaluate the real-world performance of PRS, we also conduct serious user studies by developing a Chrome extension that re-ranks the results returned by Google based on our algorithm. 
